The Graph Database Interface: Scaling Online Transactional and Analytical Graph Workloads to Hundreds of Thousands of Cores

Graph databases (GDBs) are crucial in academic and industry applications. The key challenges in developing GDBs are achieving high performance, scalability, programmability, and portability. To tackle these challenges, we harness established practices from the HPC landscape to build a system that outperforms all past GDBs presented in the literature by orders of magnitude, for both OLTP and OLAP workloads. For this, we first identify and crystallize performance-critical building blocks in the GDB design, and abstract them into a portable and programmable API specification, called the Graph Database Interface (GDI), inspired by the best practices of MPI. We then use GDI to design a GDB for distributed-memory RDMA architectures. Our implementation harnesses one-sided RDMA communication and collective operations, and it offers architecture-independent theoretical performance guarantees. The resulting design achieves extreme scales of more than a hundred thousand cores. Our work will facilitate the development of next-generation extreme-scale graph databases.

==> challenges.tex <==
\section{Challenges in Graph Databases}

We first discuss in more details challenges related to the next-generation
graph databases. 



%\maciej{Let's get the main motivation for GDI and the story.  Provide some form
%of overview of the system-design / performance / architecture of graph database
%systems, underlying problems and challenges, and making GDI the solution. How
%about...}

\subsection{Size of Datasets in Graph Databases}

%\maciej{\textbf{Challenge:} graphs used in databases are huge and will be much
%larger}
%
%\maciej{\textbf{GDI solution:} facilitates development in a distributed
%environment, focusing on how to do enable programmable, fast, and scalable data
%access and data management (sharding, ...) in extreme scales}
%
%\maciej{Describe huge industry graphs and planned ones, showing that going
%distributed (many many nodes) is the only solution, assuming we want to keep
%data in-memory (and argue why in-memory is the solution to do.)}
%
%\maciej{Add a table with such graphs, projected sizes, also in TB, etc}
%
%\maciej{We probably want to have the following details provided, but first make
%sure with Darko what can be included, also before we send it to BASF}
%
%\maciej{Some of the examples below introduce questions on appropriate models.
%Maybe we can also tell that using GDI facilitates new data models or
%query/programming models/paradigms?}


Applications require that graph databases store large graphs that might not fit into the
memory of a single machine, as shown in Table \ref{table:size}.

\if 0

\begin{table}[t]
% table data from https://arxiv.org/pdf/1904.08380.pdf
% and from https://www.cc.gatech.edu/dimacs10/downloads.shtml
% -> https://www.cc.gatech.edu/dimacs10/archive/streets.shtml

\centering
\scriptsize
\sf
\def\arraystretch{1.2}
\begin{tabular}{|l|r|r|r|}
\hline
Graph & Number of vertices |V| & Number of edges |E| & Size (GB) \\ \hline \hline
Europe (Street Network) & $50'912'018$ & $54'054'660$ & $0.864$ \\ \hline
Twitter & $41'652'231$ & $2'405'026'092$ & $38.48$ \\ \hline
ClueWeb & $978'408'098$ & $74'744'358'622$ & $1'196$ \\ \hline
Hyperlink2014 & $1'724'573'718$ & $124'141'874'032$ & $1'986$ \\ \hline
Hyperlink2012 & $3'563'602'789$ & $225'840'663'232$ & $3'613$ \\ \hline
Sogou & $\ge 271'900'000'000$ & $\ge 12'254'000'000'000$ & $\ge 136'900$ \\ \hline

\end{tabular}

\caption{Different graphs and their size when stored as list of edges (8 Byte per vertex ID),
\emph{without considering any additional data attached to vertices or edges}.} \label{table:size}
\end{table}

\fi


\begin{table*}[t]
\centering
\scriptsize
\sf
\def\arraystretch{1.2}
\begin{tabular}{c}
\hline
\multicolumn{1}{|c|}{\textbf{Layer 6: Client}} \\ \hline
A client queries the graph database.
Typically, the client uses a graph query language to
run traversals and graph matching requests.  \\ \hline \hline
                   
\multicolumn{1}{|c|}{\textbf{Layer 5: Query Planer}} \\ \hline
The query planer works in close cooperation with the execution engine
to determine an ordered set of steps to execute the 
query given by the client. \\ \hline \hline

\multicolumn{1}{|c|}{\textbf{Layer 4: Execution Engine}} \\ \hline
This layer relies on the query functions to
distribute workload among multiple machines
and aggregate intermediate results that ran on different
processes. \\ \hline \hline

\multicolumn{1}{|c|}{\textbf{Layer 3: Query Functions}} \\ \hline
This layer accesses the storage engine to provide
query functions and generic objects
to the upper layer for easier processing.
The functions typically consume data from the storage engine
and return objects like edges, vertices,
paths, or subgraphs. Aggregation functions are provided to return aggregated values.
Further functionality includes filtering of objects
(e.g. by labels or properties). \\ \hline \hline

\multicolumn{1}{|c|}{\textbf{Layer 2: Storage Engine (GDI)}} \\ \hline
This layer uses the low-level storage layer to access the graph data.
It basically translates from hardware dependent storage
to generic objects.
Therefore, the layer provides a rich set of interfaces
to create, read, update and delete (CRUD)
vertices, edges and associated labels and properties.
This layer should provide ACID guarantees to the upper layer.
If not, then a layer above must handle queries
in a way that they do not interfere. \\ \hline \hline

\multicolumn{1}{|c|}{\textbf{Layer 1: Low-Level Storage Layer (Storage Backend)}} \\ \hline
This layer provides an abstraction for a low-level
storage layer such as hard disks
(for example CSV files, JSON, binary formats, block format),
RAM, distributed RAM or others.
Its goal is to store the data in a reliable
way and provide fast data access. \\ \hline
\end{tabular}

\caption{An example layering of a graph database.  GDI is an interface for the
storage engine (layer 2).  Extensions such as query planer and execution engine
can rely on the properties that GDI offers.} \label{table:context}
\end{table*}







\subsubsection{Knowledge Graphs} \label{sec:knowledge_graph}

Knowledge graphs represent the knowledge base as a graph.
Entities, such as real world objects, people, events and abstract concepts
are represented as vertices and their relationship is modeled by edges between them.
Often the data is enriched with properties, labels, provenance information and historical data that increase the data size.
A typical use case for knowledge graphs are court hearings, where lawyers
store all data aggregated in a database and query the knowledge graph
during hearings. Such graphs must store all evidence
with additional information annotated.
Similarly, networks of people, transactions, and their relationships to companies allow to
detect money laundering and corruption scheme.
Famous examples are the Panama and Paradise papers~\cite{obermayer2016panama}.
Such applications only work efficiently when there is no restriction to add more data.
% see https://neo4j.com/blog/fighting-money-laundering-corruption-with-graph-technology/
Closely related to knowledge graphs, ontologies represent the relationship of
concepts, collected data and entities which often results in a tree-like
graph: a concept connected to an other concept closer to the root in the hierarchy indicates a
sub-concept relationship.
Since an ontology might span broad fields, the resulting graph
can contain billions of vertices and edges. Furthermore,
ontologies can always be refined and enhanced, resulting in even more growing data sizes. 



%Problem Definition:
%\begin{itemize}
%  \item bipartite graph
%  \item one partion contains documents or links to documents, no edges
%        between vertices in this partition
%  \item other partition is a tree-like hierarchy
%  \item directed edges between the two partitions indicate that a
%        particular document contains a concept from the hierarchy  
%  \item multiple hierarchies, for example chemistry with 30 million vertices
%        and hierarchy depth of 18
%  \item query: given two concepts, return the document set that is
%        created by the union of the two document sets that belong to the
%        two concepts (zero hops: perfect match, one can allow additional
%        hops in the hierarchy): matching\_query( concept1, concept2,
%        num\_hops )
%\end{itemize}
%
%\noindent Non-Technical Background:
%\begin{itemize}
%  \item 120 million patents worldwide (different validity/country, there
%        are patent families)
%  \item broad goal: query patents quickly, in the same way one would talk
%        to something like Alexa
%  \item future goal: have a word by word understanding, to completely
%        understand the documents, like for example that "this polymer"
%        references back to a specific polymer (NLP challenge in itself):
%        current system already operates at the upper limit (2.3 billion
%        vertices, some path queries take too long)
%\end{itemize}
%
%\noindent Open Questions:
%\begin{itemize}
%  \item query: restricted to just two concepts?
%  \item Is it possible to distribute the hops between the concepts?
%  \item Any additional structural information? For example: a vertex in
%        a higher position always contains edges of the vertices below
%        him?
%  \item Update model?
%\end{itemize}


\subsubsection{Protein Pathways}

Protein pathways~\cite{croft2013reactome} denote interactions between molecules in biology, that
can lead to the generation of new molecules and turn on or off genes.
Similarly, drugs can activate proteins and therefore initiate different
protein interactions. The relationship between drugs, their substance,
proteins and genomes can be represented as a graph and exceed the
available storage of a single machine, especially when the graph
is annotated with further information (e.g. details to drugs).

%Traversal queries then can easily show the effect of a drug in an
%early stage of development event without trials on subjects. 


\subsubsection{Data Modeling} \label{sec:data_modeling}

Different applications focus on data modeling and try to
represent complex real-world situations.
Examples include power providers that store their power distribution network
in a graph database, annotated with information such as the date of setup
and geographic location. The graph enables these companies to simplify planning,
track the wear of power lines,
act quickly in case
of power outages and plan actions accordingly.
Similarly, train companies can represent their rail network as graph.
A low-level representation enables not just to act appropriate in
case of an incident,
but also to plan replacements easily.
Due to the large amount of real world objects, these kind of applications
are heavily limited by graph databases that rely on a single machine.


%
%
%
%Problem Definition:
%\begin{itemize}
%  \item drugs $\rightarrow$ activate proteins $\rightarrow$ which in turn
%        initialize a cascade of reactions: called "pathway"
%  \item compare different pathways
%  \item current graph database:
%  \begin{itemize}
%    \item multiple onthologies
%    \item genome information
%    \item protein information
%    \item add product information (in the future): available drugs on
%          the market, but also ones that are currently in clinical
%          trials
%  \end{itemize}
%  \item large database
%  \item neo4j struggles with some path queries: response time too long
%\end{itemize}
%
%\noindent Non-Technical Background:
%\begin{itemize}
%  \item reactome.org
%  \item life science area
%  \item similar to Viagra, which was originally meant to be heart
%        medicine, but one of the side effects became the main marketing
%        goal
%  \item when patent expires, they want to market a different effect of
%        the same drug under a different name
%  \item compare pathways of different drugs
%\end{itemize}
%
%\noindent Open Questions:
%\begin{itemize}
%  \item What is the metric for comparing pathways?
%\end{itemize}

%skipped for now
%\subsubsection{Micro-Benchmark: Path Search Algorithm}
%
%Problem Defintion
%\begin{itemize}
%  \item from start vertex to end vertex
%  \item simple interface, but still complex in the execution (might
%        access all vertices)
%  \item path\_search( start\_vertex, end\_vertex, max\_path\_length )
%\end{itemize}

%
%\subsubsection{Power Provider (Netherlands)}
%
%Problem Definition:
%\begin{itemize}
%  \item model all single lines with a lot of attributes
%  \item in case of a powerout (temporal removal of an edge/vertex), see
%        who else is affected and find the subset for best coverage with
%        alternative lines
%\end{itemize}
%
%\noindent Open Questions:
%\begin{itemize}
%  \item How to model this? We will probably need something more complex than
%        a simple flow graph. \robert{In general, this seems to be more of
%        modeling issue than a performance issue.}
%\end{itemize}
%
%\subsubsection{Schweizer Bundesbahn}
%
%Problem Definition:
%\begin{itemize}
%  \item need 4 different levels of modeling:
%  \begin{itemize}
%    \item station/routes level (from Zurich HBF to Basel HBF for example)
%    \item tracks level
%    \item down to switches/cables detail level
%  \end{itemize}
%\end{itemize}
%
%\noindent Open Questions:
%\begin{itemize}
%  \item too much data for current graph databases according to Darko
%  \item modeling issue in general
%  \item Any upside to keeping this in one graph database or just use one
%        for each level?
%\end{itemize}

%\subsubsection{Law/Advocate}
%
%Problem Definition:
%\begin{itemize}
%  \item evidence data: currently takes a lot of human man power
%  \item goal: knowledge graph that allows for a quick look-up (during
%        trial)
%\end{itemize}

%skipped for now
%\subsubsection{Artificial Intelligence}
%
%Problem Definition:
%\begin{itemize}
%  \item How convert a graph database into a Tensor (matrix)?
%  \item possible applications: fraud detection
%  \item identify crime pattern $\rightarrow$ look for similar pattern
%  \item find abnormal pattern
%\end{itemize}


\subsection{Diversity of Workloads}


% mostly stolen from the graph database survey

Another challenge is posed by the diverse workloads that vary in the runtime, amount of touched data
and required consistency guarantee (e.g. ACID: atomicity, consistency, isolation and durability).
\emph{Online Transactional Processing (OLTP)} queries typically consist of many queries local in scope, such as
neighborhood queries, certain restricted traversals, or lookups, inserts, deletes, and updates of
single vertices and edges.
Contrarily, \emph{Offline Analytical Processing (OLAP)} workloads
are usually not processed at
interactive speed, as the queries are inherently complex and global in scope.
The LBDC benchmark \cite{ldbc} distinguish tree classes of workloads:
(1) \emph{Interactive workloads}~\cite{ldbc_interactive_paper} that can collectively be described as either read-only
queries or simple transactional updates.
(2) \emph{Business intelligence (BI)} workloads~\cite{early_ldbc_paper}
fetch large data volumes, spanning large parts of a graph. Contrarily to the
interactive workloads, the BI workloads heavily use summarization and aggregation operations
such as sorting, counting, or deriving minimum, maximum, and average values.
(3) \emph{Graph analytics benchmarks}~\cite{ldbc_graphanalytics_paper} operate on the whole graph
and exhibit long runtime. %consist of six graph algorithms that are proposed as a standard benchmark for a graph analytics
%part of a graph database.
Typically, this workload is read-only and stalls other queries since all compute resources are in use.
A different aspect to consider are \emph{Graph Pattern} and
\emph{Navigational Expression} workloads~\cite{gdb_query_language_Angles}.
Also, a common use-case is bulk input loading \cite{ciglan2012benchmarking, dominguez2010survey, jouili2013empirical}.


%\maciej{\textbf{Challenge:} Support for different aspects and classes of graph workloads:
%%
%\begin{itemize}
%%
%\item  OLTP \& OLAP;
%%
%\item LDBC three classes of workloads;
%%
%\item Property Model;
%%
%\item ACID;
%%
%\item Other stuff/keywords that people care about: traversals, pattern matching, ...
%%
%\end{itemize}
%%
%\textbf{GDI Solution:} Clear separation of concerns at the interface level? (transactions \& data access model)
%%
%Can we show how representative examples from these classes can be expressed in GDI?
%%
%}
%
%\maciej{How do we address different languages? Do we just say these are orthogonal, or shall we somehow connect
%to them more systematically?}
%
%\maciej{Do we address Turing Completeness somehow?}


\subsection{Highly-Scalable Execution}

Databases that offer scaling over many compute nodes might face
synchronization and networking overhead.



%\maciej{\textbf{Challenge:} large in-memory graphs will use many nodes.
%Performance should scale well as we go to very large scales}
%
%\maciej{\textbf{GDI Solution:} incorporation of RDMA and HPC principles
%(collective communication, what else specifically?)}

% skipped for now - they know that Neo4j etc is slow
%\subsection{Analysis of the State-Of-The-Art}
%
%\maciej{We could compress the survey into a small table here, that lists
%different graph databases and shows if they support all these aspects above,
%showing clearly no solution does that fully? Then argue that GDI on its own can
%\textbf{enable} these systems to reach these goals, and also show that NOD is a
%reference implementation that \textbf{enables that for specific classes of
%queries}?}


\subsection{Low-Latency Execution}

Response time is crucial for customer satisfaction and graph
da\-ta\-bases must serve a large number of concurrent users.
Such use cases include incident management and processing knowledge graphs,
as outlined in Section \ref{sec:knowledge_graph} and \ref{sec:data_modeling}.

%\maciej{\textbf{Challenge:} Different workloads must be high-performance,
%namely low latency and high throughput.}
%
%\maciej{\textbf{GDI Solution:} blocked data layer on top of fast RDMA enabled
%memories.}


\subsection{Portability}

It is crucial for databases to support different systems
like cloud platforms, HPC data centers and desktop systems.
GDI offers this functionality since it just specifies an interface and makes
no other assumptions about the underlying implementation.
This layering enables implementing system specific GDI software %that
% exploits possible hardware acceleration function
for highest performance.
Libraries (such as query planers, execution engines or graph languages)
that rely on GDI can simply switch to a different compute system with a different GDI
implementation without the need for re-implementation.


%
%\maciej{\textbf{Challenge:} One should be able to run a database on top of
%different systems and machines}
%
%\maciej{\textbf{GDI Solution:} we surely do a reference implementation for Cray
%systems, but the whole idea is to make GDI system agnostic, and ensure
%portability. Can we claim the same for the blocked data access layer design? We
%can claim that blocked data depends on the RMA semantics, which are also
%independent of the details of RDMA implementation, and thus the blocked data
%design it is portable across any systems that have these semantics (iWARP,
%RoCE, shared memories, etc?)}





==> gdi-list-table.tex <==
\begin{table*}[t]
\vspaceSQ{-1em}
\centering
\setlength{\tabcolsep}{2pt}
%\sf
\footnotesize
\scriptsize
%
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
%
\makecell[c]{\textbf{Routines}} & 
\makecell[c]{\textbf{Description}} & 
\makecell[c]{\textbf{Type}} & 
\makecell[c]{\textbf{Tr}} & 
\makecell[c]{\textbf{oTr}} & 
\makecell[c]{\textbf{Work}} & 
\makecell[c]{\textbf{Depth}} \\
%
\midrule
%
\multicolumn{7}{l}{\textcolor{gray}{\textbf{General management (setup to be performed before other GDI functions may be called)}}} \\
%
\midrule
%
\texttt{GDI\_Init} & Allocate all necessary internal data structures that are needed by GDI & C & no & yes & $O(P)$ & $O(\log P)$ \\
\texttt{GDI\_Finalize} & Deallocate all internal data structures and any remaining graph database objects & C & no & yes &  $O(P)$ & $O(\log P)$ \\
\texttt{GDI\_CreateDatabase,  GDI\_FreeDatabase} & Create or deallocate a database object and all the related structures & C & no & yes &  $O(P)$ & $O(\log P)$ \\
%
\midrule
%
\multicolumn{7}{l}{\textcolor{blue}{\textbf{CRUD routines for graph metadata (labels, property types)}}} \\
%
\midrule
%
\texttt{GDI\_CreateLabel, GDI\_UpdateLabel, GDI\_FreeLabel} & Create, update, or deallocate a label object & C & no & yes & $O(P)$ & $O(\log P)$ \\
\texttt{GDI\_GetLabelFromName, GDI\_GetNameOfLabel} & Return a label object based on a name, or get the name of a label object & L & yes & yes & $O(1)$ & $O(1)$ \\
\texttt{GDI\_GetAllLabelsOfDatabase} & Return all the labels associated with a given database & L & yes & yes & $O(|\mathcal{L}|)$ & $O(1)$ \\
\texttt{GDI\_CreatePType, GDI\_UpdatePType, GDI\_FreePType} & Create, update, and deallocate a property type object & C & no & yes & $O(P)$ & $O(\log P)$ \\
\texttt{GDI\_GetPTypeFromName, GDI\_GetNameOfPType} & Return a property type object based on a name, get a property type's name & L & yes & yes & $O(1)$ & $O(1)$ \\
\texttt{GDI\_GetAllPTypesOfDatabase} & Return all the property types associated with a given database & L & yes & yes & $O(|\mathcal{P}|)$ & $O(1)$ \\ 
\texttt{GDI\_GetEntityTypeOfPType, GDI\_GetDatatypeOfPType, GDI\_GetSizeLimitOfPType} & Query different aspects of a property type & L & yes & yes & $O(1)$ & $O(1)$ \\
%
\midrule
%
\multicolumn{7}{l}{\textcolor{cyan}{\textbf{CRUD routines for graph data (vertices, edges, and their attached labels and properties)}}} \\
%
\if 0
\midrule
%
\texttt{GDI_CreateVertex, GDI_FreeVertex} & Create or deallocate a vertex object
\texttt{GDI_GetEdgesOfVertex, GDI_GetNeighborVerticesOfVertex} & Return adjacent edges or vertices (of a given vertex)
\texttt{GDI_AddLabelToVertex, GDI_RemoveLabelFromVertex}
\texttt{}
\texttt{}
\texttt{}
%
\midrule
%
\multicolumn{7}{l}{\textcolor{green}{\textbf{Transactional processing of graph data}}} \\
%
\midrule
%
\texttt{}
\texttt{}
\texttt{}
\texttt{}
%
\midrule
%
\multicolumn{7}{l}{\textcolor{orange}{\textbf{Indexing structures for accelerating queries on graph data}}} \\
%
\midrule
%
\texttt{}
\texttt{}
\texttt{}
\texttt{}
\texttt{}
%
\midrule
%
\multicolumn{7}{l}{\textcolor{brick}{\textbf{Constraints defining the conditions for indexing}}} \\
%
\midrule
%
\texttt{}
\texttt{}
\texttt{}
\texttt{}
\texttt{}
\texttt{}
\texttt{}
%
%
\fi
\bottomrule
%
\end{tabular}
%}
%\vspaceSQ{-0.5em}
%
\caption{Selected most important GDI routines and the fundamental performance of our
corresponding GDI-RMA implementation.
%
``\ul{Type}'': local (L) or collective (C).
%
``\ul{Tr}'': can it be executed within a transaction?
%
``\ul{oTr}'': can it be executed outside a transaction?
%
``\ul{Work}'': the total amount of operations in a parallel execution.
%
``\ul{Depth}'': the longest sequential chain of dependencies (i.e., the
sequential botleneck) in a parallel execution.
%
}
%
\vspaceSQ{-1.5em}
\label{tab:gdi-listing}
%
\end{table*}






==> gdi-listing.tex <==
%\begin{minipage}[c]{\textwidth}
%
% \begin{lstlisting}[float=*hbtp, captionpos=t, abovecaptionskip=-1em, backgroundcolor=\color{llgrey}, title=Most important GDI routines related to: general management (\textcolor{gray}{\textbf{gray color}}), graph metadata (\textcolor{blue}{\textbf{blue color}}), graph data (\textcolor{cyan}{\textbf{cyan color}}), indexes (\textcolor{orange}{\textbf{orange color}}), transactions (\textcolor{green}{\textbf{green color}}), and constraints (\textcolor{brick}{\textbf{brick red color}})., label=lst:gdi-general]
%
\begin{lstlisting}[float=*t, captionpos=t, abovecaptionskip=-1em, backgroundcolor=\color{llgrey}, title=Most important GDI routines related to: general management (\textcolor{gray}{\textbf{gray color}})\mbox{,} graph metadata (\textcolor{blue}{\textbf{blue color}})\mbox{,} graph data (\textcolor{cyan}{\textbf{cyan color}})\mbox{,} indexes (\textcolor{orange}{\textbf{orange color}})\mbox{,} transactions (\textcolor{green}{\textbf{green color}})\mbox{,} and constraints (\textcolor{brick}{\textbf{brick red color}})., label=lst:gdi-general]
[C] GDI_Init //Allocate all necessary internal data structures that are needed by GDI.
[C] GDI_Finalize //Deallocate all internal data structures and any remaining graph database objects.
[C] GDI_CreateDatabase / GDI_FreeDatabase //Create / deallocate a database object and all the related structures
\end{lstlisting} 
%
\begin{lstlisting}[float=*t, captionpos=t, aboveskip=-1.5em, backgroundcolor=\color{llblue}, label=lst:gdi-metadata]
[C] GDI_CreateLabel, GDI_UpdateLabel, GDI_FreeLabel //Create, update, or deallocate a label object
[L] GDI_GetLabelFromName, GDI_GetNameOfLabel //Return a label object based on a name, get the name of a label object
[L] GDI_GetAllLabelsOfDatabase //Return all the labels associated with a given database
[C] GDI_CreatePropertyType, GDI_UpdatePropertyType, GDI_FreePropertyType //Create, update, and deallocate a property type object
[L] GDI_GetPropertyTypeFromName, GDI_GetNameOfPropertyType //Return a property type object based on a name, get a property type's name
[L] GDI_GetAllPropertyTypesOfDatabase //Return all the property types associated with a given database
[L] GDI_GetEntityTypeOfPropertyType, GDI_GetDatatypeOfPropertyType, GDI_GetSizeLimitOfPropertyType //Query aspects of a property type
\end{lstlisting}
%
\begin{lstlisting}[float=*t, captionpos=t, aboveskip=-1.5em, backgroundcolor=\color{llred}, label=lst:gdi-data]
[L] GDI_CreateVertex, GDI_FreeVertex //Create or deallocate a vertex object 
[L] GDI_GetEdgesOfVertex, GDI_GetNeighborVerticesOfVertex //Return adjacent edges or vertices (of a given vertex)
[L] GDI_AddLabelToVertex, GDI_RemoveLabelFromVertex, GDI_GetAllLabelsOfVertex, GDI_AddPropertyToVertex, GDI_UpdatePropertyOfVertex, GDI_SetPropertyOfVertex, GDI_RemovePropertyFromVertex, GDI_RemovePropertiesFromVertex, GDI_GetPropertiesOfVertex, GDI_GetAllPropertyTypesOfVertex //CRUD routines for labels, properties, and property types of a given specific vertex object
[L] GDI_CreateEdge, GDI_FreeEdge //Create a new edge as well as an access object during a transaction
[L] GDI_GetVerticesOfEdge, GDI_GetDirectionTypeOfEdge, GDI_SetOriginVertexOfEdge, GDI_SetTargetVertexOfEdge, GDI_SetDirectionTypeOfEdge
[L] GDI_AddLabelToEdge, GDI_RemoveLabelFromEdge, GDI_GetAllLabelsOfEdge, GDI_AddPropertyToEdge, GDI_GetAllPropertyTypesOfEdge, GDI_GetPropertiesOfEdge, GDI_RemovePropertiesFromEdge, GDI_RemoveSpecificPropertyFromEdge, GDI_UpdatePropertyOfEdge, GDI_UpdateSpecificPropertyOfEdge, GDI_SetPropertyOfEdge //CRUD routines for labels, properties, and property types of a given edge
[L] GDI_AssociateVertex, GDI_AssociateEdge //Create an access object (handle) during a transaction for an existing vertex or edge.
\end{lstlisting}
%
\begin{lstlisting}[float=*t, captionpos=t, aboveskip=-1.5em, backgroundcolor=\color{llgreen}, label=lst:gdi-indexes]
[C] GDI_CreateIndex, GDI_FreeIndex //Create or deallocate an index 
[C] GDI_AddLabelToIndex, GDI_RemoveLabelFromIndex, GDI_AddPropertyTypeToIndex, GDI_RemovePropertyTypeFromIndex, GDI_AddLabelsAndPropertyTypesToIndex, GDI_RemoveLabelsAndPropertyTypesFromIndex, GDI_GetAllLabelsOfIndex, GDI_GetAllPropertyTypesOfIndex //Some of CRUD routines for conditioning a given index with labels and property types
[L] GDI_TranslateVertexID //Retrieve a vertex using a given label and an application-level ID
[L] GDI_GetVerticesOfIndex, GDI_GetEdgesOfIndex //Retrieve all vertices / edges from the index object that satisfy the constraint
[L] GDI_GetLocalVerticesOfIndex, GDI_GetLocalEdgesOfIndex //Retrieve all vertices / edges from the index object that satisfy the constraint, and which are also local to the calling process
[L] GDI_GetTypeOfIndex //Return the specific implementation type of a given index
\end{lstlisting}
%
\begin{lstlisting}[float=*t, captionpos=t, aboveskip=-1.5em, backgroundcolor=\color{llblue}, label=lst:gdi-transactions]
[L] GDI_StartTransaction, GDI_CloseTransaction //Start or commit a single-process transaction
[C] GDI_StartCollectiveTransaction, GDI_CloseCollectiveTransaction //Start or commit a collective transaction
[L] GDI_GetAllTransactionsOfDatabase //Retrieve handles to all ongoing transactions
[L] GDI_GetTypeOfTransactio //Retrieve the type of a given ongoing transaction 
\end{lstlisting}
%
\begin{lstlisting}[float=*t, captionpos=t, aboveskip=-2.5em, backgroundcolor=\color{llyellow}, label=lst:gdi-constraints]
[L] GDI_CreateConstraint, GDI_FreeConstraint, GDI_CreateSubconstraint, GDI_FreeSubconstraint //Create or deallocate constraint objects, used in indexes 
[L] GDI_AddLabelConditionToSubconstraint, GDI_AddPropertyConditionToSubconstraint //Extend constraints with new conditions
[L] GDI_AddSubconstraintToConstraint //Extend a constraint with a subconstraint
[L] GDI_GetAllConstraintsOfDatabase, GDI_GetAllSubconstraintsOfConstraint //Retrieve all constraints or subconstraints
[L] GDI_IsConstraintStale, GDI_IsSubconstraintStale //Check the staleness of constraints or subconstraints
[L] GDI_GetAllLabelConditionsFromSubconstraint, GDI_GetAllPropertyTypesOfSubconstraint, GDI_GetPropertyConditionsOfSubconstraint //Retrieve label or property type conditions from given constraints
\end{lstlisting}
%
%[L] int GDI_GetLocalVerticesOfIndex(); //Retrieve all vertices from the index object that satisfy the constraint and are local to the process (same parameter list as GDI_GetVerticesOfIndex)
%[L] int GDI_GetEdgesOfIndex( GDI_Edge_uid array_of_uids[], size_t count, size_t* resultcount, GDI_Constraint constraint, GDI_Index index, GDI_Transaction transaction ); //Retrieve all edges from the index object that satisfy the constraint
%[L] int GDI_GetLocalEdgesOfIndex( GDI_Edge_uid array_of_uids[], size_t count, size_t* resultcount, GDI_Constraint constraint, GDI_Index index, GDI_Transaction transaction ); //Retrieve all edges from the index object that satisfy the constraint and are local to the process
%
%\end{minipage}

\if 0

% Mac comment: stuff below comes with all extensive parameter lists

\begin{lstlisting}[float=*t, caption=The most important functions included in GDI; \mbox{``[C]''} and \mbox{``[L]''} indicate a collective and non-collective call\mbox{,} respectively., label=lst:gdi]
//|\textbf{\ul{GDI initialization / completion}}|: setup to be performed before other GDI functions may be called. 
[C] int GDI_Init( int *argc, char ***argv ); //Allocate all necessary internal data structures that are needed by GDI.
|\vspace{0.5em}|[C] int GDI_Finalize(); //Deallocate all internal data structures and any remaining graph database objects.
//|\textbf{\ul{Database management}}|: general management; |db|: a pointer to a database object, |params|: any input parameters required by a given database.
[C] int GDI_CreateDatabase( void* params, size_t params_size, GDI_Database* db ); //Create a database object and all the needed structures
|\vspace{0.5em}|[C] int GDI_FreeDatabase( GDI_Database* db ); //Deallocate a database |db| and all structures associated with it
//|\textbf{\ul{Graph metadata}}|: management of label & property type objects; |db|: a pointer to a database, |label|: a pointer to a label, |name|: a label name, |ptype|: a pointer to a property type, , 
[C] int GDI_CreateLabel( const char* name, GDI_Database db, GDI_Label* label ); //Create a label object
[C] int GDI_FreeLabel( GDI_Label* label ); //Deallocate the given label object and remove it from all vertices and edges
[C] int GDI_CreatePropertyType( const char* name, int etype, GDI_Datatype dtype, int stype, size_t count, GDI_Database db, GDI_PropertyType* ptype ); //Create a property type object, etype and stype specify possible limitations of the property type
[C] int GDI_FreePropertyType( GDI_PropertyType* ptype ); //Deallocate the given property type object and remove all properties with that type from all vertices and edges
|\vspace{0.5em}|[C] int GDI_UpdatePropertyType( const char* name, int etype, GDI_Datatype dtype, int stype, size_t count, const void* default_value, GDI_PropertyType ptype ); //Update the limitations, possibly updates all vertex and edge properties of that property type
//|\textbf{\ul{Indexes}}|: management and retrieval from index objects
[C] int GDI_CreateIndex( size_t obj_count, int itype, GDI_Database db, GDI_Index* index ); //Create an index object and all needed structures, itype specifies an implementation hint (hashtable/B-Tree)
[C] int GDI_FreeIndex( GDI_Index* index ); //Deallocates all structures as well as the given index object
[C] int GDI_AddLabelsAndPropertyTypesToIndex( GDI_Label array_of_labels[], size_t label_count, GDI_PropertyType array_of_ptypes[], size_t ptype_count, GDI_Index index ); //Add labels and property types to the index object, so that vertices and edges with the respective labels and properties of those types are indexed
[C] int GDI_RemoveLabelsAndPropertyTypesFromIndex( GDI_Label array_of_labels[], size_t label_count, GDI_PropertyType array_of_ptypes[], size_t ptype_count, GDI_Index index ); //Remove labels and property types from the index object, might require a rebuilding of the index
[L] int GDI_TranslateVertexID( bool* found_flag, GDI_Vertex_uid* internal_uid, GDI_Label label, const void* external_id, size_t size, GDI_Transaction transaction ); //Retrieve vertex with the given label and application-level ID, index over GDI_PROPERTY_TYPE_ID
[L] int GDI_GetVerticesOfIndex( GDI_Vertex_uid array_of_uids[], size_t count, size_t* resultcount, GDI_Constraint constraint, GDI_Index index, GDI_Transaction transaction ); //Retrieve all vertices from the index object that satisfy the constraint
[L] int GDI_GetLocalVerticesOfIndex( GDI_Vertex_uid array_of_uids[], size_t count, size_t* resultcount, GDI_Constraint constraint, GDI_Index index, GDI_Transaction transaction ); //Retrieve all vertices from the index object that satisfy the constraint and are local to the process

|\textbf{// \ul{Transactions}}|: starting, completion, and abortion of transactions
[L] int GDI_StartTransaction( GDI_Database db, GDI_Transaction* transaction ); //Start a transaction
[L] int GDI_CloseTransaction( GDI_Transaction* transaction, int ctype ); //End a transaction, ctype specifies whether to commit or abort
[C] int GDI_StartCollectiveTransaction( GDI_Database db, GDI_Transaction* transaction ); //Start a collective transaction 
[C] int GDI_CloseCollectiveTransaction( GDI_Transaction* transaction, int ctype ); //End a transaction, ctype specifies whether to commit or abort

|\textbf{// \ul{Graph data}}|: adding and removing vertices, edges, labels, and properties
[L] int GDI_CreateVertex( const void* external_id, size_t size, GDI_Transaction transaction, GDI_VertexHolder* vertex ); //Create a new vertex as well as an access object during a transaction, external_id specifies the application-level ID, a property, of the vertex
[L] int GDI_GetEdgesOfVertex( GDI_Edge_uid array_of_uids[], size_t count, size_t* resultcount, GDI_Constraint constraint, int edge_orientation, GDI_VertexHolder vertex ); //Retrieve incident edges of vertex, edge_orientation is a combination of incoming, outgoing and undirected
[L] int GDI_CreateEdge( int dtype, GDI_VertexHolder origin, GDI_VertexHolder target, GDI_EdgeHolder* edge ); //Create a new edge as well as an access object during a transaction, dtype specifies whether the edge is directed or undirected
[L] int GDI_GetVerticesOfEdge( GDI_Vertex_uid* origin_uid, GDI_Vertex_uid* target_uid, GDI_EdgeHolder edge ); //Retrieve vertices incident to the edge
// similar functionalities to the ones below also exist for edges
[L] int GDI_FreeVertex( GDI_VertexHolder* vertex ); //Deallocation of the access object and removal of the vertex from the database
[L] int GDI_AssociateVertex( GDI_Vertex_uid internal_uid, GDI_Transaction transaction, GDI_VertexHolder* vertex ); //Creation of an access object during a transaction for an existing vertex
[L] int GDI_AddLabelToVertex( GDI_Label label, GDI_VertexHolder vertex ); //Add label to vertex
[L] int GDI_RemoveLabelFromVertex( GDI_Label label, GDI_VertexHolder vertex ); //Remove label from vertex
[L] int GDI_GetAllLabelsOfVertex( GDI_Label array_of_labels[], size_t count, size_t* resultcount, GDI_VertexHolder vertex ); //Retrieve labels of vertex
[L] int GDI_AddPropertyToVertex( const void* value, size_t count, GDI_PropertyType ptype, GDI_VertexHolder vertex ); //Add property to vertex
[L] int GDI_RemovePropertiesFromVertex( GDI_PropertyType ptype, GDI_VertexHolder vertex ); //Remove all properties of type ptype from the vertex
[L] int GDI_GetPropertiesOfVertex( void* buf, size_t buf_count, size_t* buf_resultcount, size_t array_of_offsets[], size_t offset_count, size_t* offset_resultcount, GDI_PropertyType ptype, GDI_VertexHolder vertex ); //retrieve property values of the properties with type ptype from vertex

|\textbf{// \ul{Constraints}}|:
[L] int GDI_CreateConstraint( GDI_Database db, GDI_Constraint* constraint ); //Create a constraint object
[L] int GDI_FreeConstraint( GDI_Constraint* constraint ); //Deallocate the given constraint object
[L] int GDI_CreateSubconstraint( GDI_Database db, GDI_Subconstraint* subconstraint ); //Create a subconstraint object
[L] int GDI_FreeSubconstraint( GDI_Subconstraint* subconstraint ); //Deallocate the given subconstraint object
[L] int GDI_AddLabelConditionToSubconstraint( GDI_Label label, GDI_Op op, GDI Subconstraint subconstraint ); //Object has or has not label
[L] int GDI_AddPropertyConditionToSubconstraint( GDI_PropertyType ptype, GDI_op op, void* value, size_t count, GDI_Subconstraint subconstraint ); //Add a property condition to the subconstraint object
[L] int GDI_AddSubconstraintToConstraint( GDI_Subconstraint subconstraint, GDI_Constraint constraint ); //Add a subconstraint to the constraint object
\end{lstlisting}

\fi


==> scale.tex <==
\section{Towards 100,000 Cores and Beyond}

